Dynamic Mesh-Aware Radiance Fields

Embedding polygonal mesh assets within photorealistic Neural Radience Fields (NeRF) volumes, such that they can be rendered and their dynamics simulated in a physically consistent manner with the NeRF, is under-explored from the system perspective of integrating NeRF into the traditional graphics pipeline. This paper designs a two-way coupling between mesh and NeRF during rendering and simulation. We first review the light transport equations for both mesh and NeRF, then distill them into an efficient algorithm for updating radiance and throughput along a cast ray with an arbitrary number of bounces. To resolve the discrepancy between the linear color space that the path tracer assumes and the sRGB color space that standard NeRF uses, we train NeRF with High Dynamic Range (HDR) images. We also present a strategy to estimate light sources and cast shadows on the NeRF. Finally, we consider how the hybrid surface-volumetric formulation can be efficiently integrated with a high-performance physics simulator that supports cloth, rigid and soft bodies. The full rendering and simulation system can be run on a GPU at interactive rates. We show that a hybrid system approach outperforms alternatives in visual realism for mesh insertion, because it allows realistic light transport from volumetric NeRF media onto surfaces, which affects the appearance of reflective/refractive surfaces and illumination of diffuse surfaces informed by the dynamic scene.

==> shortcut.tex <==
\usepackage{times}
\usepackage{epsfig}
\usepackage{graphicx}
\usepackage{float}
\usepackage{wrapfig}
\usepackage{amsmath,amsthm}
\usepackage{graphicx}

\makeatletter
\newsavebox\myboxA
\newsavebox\myboxB
\newlength\mylenA

\newcommand*\xoverline[2][0.75]{%
    \sbox{\myboxA}{$\m@th#2$}%
    \setbox\myboxB\null% Phantom box
    \ht\myboxB=\ht\myboxA%
    \dp\myboxB=\dp\myboxA%
    \wd\myboxB=#1\wd\myboxA% Scale phantom
    \sbox\myboxB{$\m@th\overline{\copy\myboxB}$}%  Overlined phantom
    \setlength\mylenA{\the\wd\myboxA}%   calc width diff
    \addtolength\mylenA{-\the\wd\myboxB}%
    \ifdim\wd\myboxB<\wd\myboxA%
       \rlap{\hskip 0.5\mylenA\usebox\myboxB}{\usebox\myboxA}%
    \else
        \hskip -0.5\mylenA\rlap{\usebox\myboxA}{\hskip 0.5\mylenA\usebox\myboxB}%
    \fi}
\makeatother

\usepackage{bm,xspace}
\usepackage{comment}
\usepackage{verbatim}
\usepackage{multirow}
\usepackage{balance}
\usepackage{url}
\usepackage{booktabs}
\usepackage{etoolbox,siunitx}
\usepackage{calc}
\usepackage{pifont,hologo}
\setlength\heavyrulewidth{0.10em}
\setlength\lightrulewidth{0.05em}
\setlength\cmidrulewidth{0.03em}
\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}
% \usepackage{algpseudocode}

\usepackage[super]{nth}
\usepackage{nicefrac}
\sisetup{detect-weight=true,detect-inline-weight=math}
\sisetup{quotient-mode = fraction}
\sisetup{fraction-function = \nicefrac}
\robustify\bfseries


\def\aa{\mathbf{a}}
\def\bb{\mathbf{b}}
\def\cc{\mathbf{c}}
\def\dd{\mathbf{d}}
\def\ee{\mathbf{e}}
\def\ff{\mathbf{f}}
\def\gg{\mathbf{g}}
\def\hh{\mathbf{h}}
\def\ii{\mathbf{i}}
\def\jj{\mathbf{j}}
\def\kk{\mathbf{k}}
\def\ll{\mathbf{l}}
\def\mm{\mathbf{m}}
\def\nn{\mathbf{n}}
\def\oo{\mathbf{o}}
\def\pp{\mathbf{p}}
\def\qq{\mathbf{q}}
\def\rr{\mathbf{r}}
\def\sss{\mathbf{s}}
\def\tt{\mathbf{t}}
\def\uu{\mathbf{u}}
\def\vv{\mathbf{v}}
\def\ww{\mathbf{w}}
\def\xx{\mathbf{x}}
\def\yy{\mathbf{y}}
\def\zz{\mathbf{z}}

\def\AA{\mathbf{A}}
\def\BB{\mathbf{B}}
\def\CC{\mathbf{C}}
\def\DD{\mathbf{D}}
\def\EE{\mathbf{E}}
\def\FF{\mathbf{F}}
\def\GG{\mathbf{G}}
\def\HH{\mathbf{H}}
\def\II{\mathbf{I}}
\def\JJ{\mathbf{J}}
\def\KK{\mathbf{K}}
\def\LL{\mathbf{L}}
\def\MM{\mathbf{M}}
\def\NN{\mathbf{N}}
\def\OO{\mathbf{O}}
\def\PP{\mathbf{P}}
\def\QQ{\mathbf{Q}}
\def\RR{\mathbf{R}}
\def\SS{\mathbf{S}}
\def\TT{\mathbf{T}}
\def\UU{\mathbf{U}}
\def\VV{\mathbf{V}}
\def\WW{\mathbf{W}}
\def\XX{\mathbf{X}}
\def\YY{\mathbf{Y}}
\def\ZZ{\mathbf{Z}}

\def\aA{\mathcal{A}}
\def\bB{\mathcal{B}}
\def\cC{\mathcal{C}}
\def\dD{\mathcal{D}}
\def\eE{\mathcal{E}}
\def\fF{\mathcal{F}}
\def\gG{\mathcal{G}}
\def\hH{\mathcal{H}}
\def\iI{\mathcal{I}}
\def\jJ{\mathcal{J}}
\def\kK{\mathcal{K}}
\def\lL{\mathcal{L}}
\def\mM{\mathcal{M}}
\def\nN{\mathcal{N}}
\def\oO{\mathcal{O}}
\def\pP{\mathcal{P}}
\def\qQ{\mathcal{Q}}
\def\rR{\mathcal{R}}
\def\sS{\mathcal{S}}
\def\tT{\mathcal{T}}
\def\uU{\mathcal{U}}
\def\vV{\mathcal{V}}
\def\wW{\mathcal{W}}
\def\xX{\mathcal{X}}
\def\yY{\mathcal{Y}}
\def\zZ{\mathcal{Z}}

\def\Ae{\mathbb{A}}
\def\Be{\mathbb{B}}
\def\Ce{\mathbb{C}}
\def\Le{\mathbb{L}}
\def\Ne{\mathbb{N}}
\def\Pe{\mathbb{P}}
\def\Qe{\mathbb{Q}}
\def\Re{\mathbb{R}}
\def\Se{\mathbb{S}}
\def\Te{\mathbb{T}}
\def\Xe{\mathbb{X}}
\def\Ye{\mathbb{Y}}
\def\Ze{\mathbb{Z}}

\def\btheta{{\bm\theta}}
\def\bzeta{{\bm\zeta}}
\def\bmu{{\bm\mu}}
\def\bZero{\mathbf{0}}
\def\bOne{\mathbf{1}}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\minimize}{minimize}
\DeclareMathOperator*{\maximize}{minimize}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\trace}{tr}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\diam}{diam}

\def\eps{\varepsilon}
\def\vphi{\varphi}
\def\vsigma{\varsigma}

\def\trans{^{\top}}
\def\deg{^{\circ}}

\def\th{^{\textnormal{th}}}
\def\st{^{\textnormal{st}}}
\def\nd{^{\textnormal{nd}}}

\newcommand\ggreater{\mathbin{>\!\!\!>}}
\newcommand\llesser{\mathbin{<\!\!\!<}}

\newcommand{\YesV}{\ding{51}}%
\newcommand{\NoX}{\ding{55}}
\DeclareMathSymbol{@}{\mathord}{letters}{"3B}

\newcommand\paren[1]{\left(#1\right)}
\newcommand\abs[1]{\left\lvert#1\right\rvert}
\newcommand\norm[1]{\left\lVert#1\right\rVert}
\newcommand\tuple[1]{\left\langle#1\right\rangle}
\newcommand\inner[2]{\langle #1, #2 \rangle}


\newcommand\crossb[1]{[#1]_\times}


\newcommand\timess{\mathbin{\!\times\!}}

\newcommand\nicebar[1]{\mkern 4mu\overline{\mkern-4mu#1}}

\newcommand\yourname[1]{\textcolor{blue}{Name says: #1}}

\newcommand\mypara[1]{\vspace{1mm}\noindent\textbf{#1}}

\def\rot#1{\rotatebox{90}{#1}}

\def\latex/{\LaTeX}
\def\bibtex/{\hologo{BibTeX}}


% \newcommand\PD[2]{\frac{\partial #1}{\partial #2}}
\newcommand\adj[2]{\overline{ #1}_{#2}}

==> tex/coverletter.tex <==
\section{Cover Letter}
This work was first submitted to SIGGRAPH 2023, we thank the reviewers for their recognition ``It is an interesting idea to combine NeRF-based ray marching with traditional ray-tracing"; ``It's the first time seeing the rendering of transparent/reflective media together with NeRFs". At the same time, reviewers also point out that the motivation and contribution should be made clearer; there should be more literature review for volume rendering; NeRF should be influenced by mesh; the difference between sRGB space of NeRF and linear RGB space for pace tracer should be handled during rendering.



% The motivation for this work is a bit puzzling as it is based on the fl awed assumption that it is "unclear how tobest incorporate NeRF's volumetric scene representations with widely adopted traditional graphics pipelines"[L90].

% In this submission, we improve our previous methods in the following aspects.

Based on the reviewers' constructive feedback, the following changes are mode,
%\vspace{-\topsep}
\begin{itemize}
\setlength{\itemsep}{1mm}
\setlength{\parskip}{0pt}
    \item We correct inaccurate description, complete missing definition, review more related literature, changing citation style, etc.
    \item We add support for HDR data which can unify the color space of the path tracer and NeRF. 
    \item We modify the NeRF rendering equation and query secondary rays during path-tracing to cast shadows on NeRF.
    \item  We use a differentiable surface rendering~\cite{Mitsuba3} to estimate light sources from the environment.
    \item We made the NeRF also dynamic in simulation so there is two-way coupling between NeRF and mesh.
\end{itemize}

\subsection{Writing}
Volume rendering has a long history. Great progress and impressive visual results have been witnessed in the recent years.
We review more recent literature on rendering participating media ~\cite{muller16efficient,miller19null,novak14thesis,Novak18volumeSTAR}. Instead of proposing a totally new volume rendering method, we define the scope of our contribution to be integrating the recent popular Neural Radiance Fields (NeRF) into this big pipeline. We are focusing on improving the two-way coupling between mesh and NeRF (reflections, shadows, simulation, etc.) and make the system efficient and user-friendly.

Moreover, we have corrected typos, undefined symbols, and inaccurate descriptions.


\subsection{HDR Rendering}
It was pointed out that ``NeRFs perform ray marching in sRGB. From a physical point of view that is fairlymeaningless but it works. The path tracer on the other hand should be using linear RGB".

The standard NeRF model accumulates sRGB color along rays cast from the camera into the volume: each point's color is represented by three 8-bit values, one for each color channel.  Integrating these colors along the ray (weighted by transmittance) produces a final 8-bit color value, the rendered pixel color, which is compared to the corresponding ground truth 8-bit pixel color to supervise NeRF training.

In contrast, path tracing assumes radiance values are expressed in linear color space.  In order to relate NeRF and surface rendering in a physically meaningful way, they should ideally operate in a common color space.  To reconcile this difference, we train an HDR variant of NeRF, supervised with 32-bit HDR images directly rather than the standard 8-bit NeRF.  The resulting HDR NeRF produces a 3-channel radiance $L_i(p, \omega$ in 32-bit \textit{linear color space} at each sampled point.  

The HDR NeRF rendering equation can thus be written as:
\begin{equation}
\label{eq:hdr_nerf_cl}
    L_i(p, \omega) = \int_{0}^{t_f} T(t)\sigma(p_t) L_i(p_t, \omega) dt
\end{equation}
where the transmittance term $T(t)$ remains unchanged.  The sRGB value can be computed by $r(p, \omega) = \psi(L_i(p,\omega))$, where $\psi(\cdot)$ represents a tone-mapping function from linear to sRGB color space. We refer interested readers to \cite{mildenhall2022rawnerf} for a deep dive about HDR NeRF.  

With this simple adjustment, the NeRF equation can now be related directly to the surface rendering equation.  If it is impractical to capture HDR training data, one can still use standard (LDR) NeRF. In this case, since the NeRF volume acts as the only light source, and the total energy is dissipative during the light transport, $L_i(p, \omega)$ will never exceed the NeRF volume's maximal radiance.  $\psi(\cdot)$ would then degenerate to an identity mapping such that $L(p, \omega) = r(p, \omega)$.  In other words, in many practical cases, reasonable visual results could still be obtained if standard NeRF is used with our system, despite the resulting inaccuracy in the light transport simulation.


\begin{figure}
\centering
\begin{tabular}{@{}c@{\hspace{1mm}}c@{\hspace{1mm}}c@{\hspace{1mm}}c@{}}
    \includegraphics[width=0.25\linewidth]{figure/hdr_1.png} &
    \includegraphics[width=0.25\linewidth]{figure/ldr_1.png} &
    \includegraphics[width=0.25\linewidth]{figure/hdr_2.png} &
    \includegraphics[width=0.25\linewidth]{figure/ldr_2.png} \\
    \small (a) HDR & \small (c) LDR  &
    \small (b) HDR [-3.5 EV] & \small (d) LDR [-1.5 EV] \\
\end{tabular}
\vspace{-1em}
\caption{\textbf{HDR Volumetric Radiance Map.} The diffuse sphere is rendered using our hybrid algorithm.  Images rendered using the NeRF trained in 32-bit HDR (a, b) achieve a higher level of lighting realism than those rendered with 8-bit LDR (c, d).}
\label{fig:comp_hdr_cl}
\vspace{-1em}
\end{figure}


\mypara{Rendering with HDR NeRF.}
We provide a preliminary qualitative comparison between rendering using the standard (LDR) NeRF and its HDR counterpart, shown in Figure~\ref{fig:comp_hdr_cl}.  Notice that in the images rendered with the HDR model, the lighting cast from the environment onto the mesh appears much more faithful to the scene's true intensity (and therefore directionality).  This is also not surprising, considering the longstanding use of High Dynamic Range Image-Based Lighting in the traditional graphics pipeline \cite{debevec_hdr_ibl}.  HDR images are often created by recovering the unknown nonlinear tone-mapping function from a series of bracketed-exposure LDR images with known exposure duration, then using the inverse function to map the images back to linear color space, and merging them into a single 32-bit result, as introduced by Debevec and Malik in 1997 \cite{debevec1997}.  As a result, HDR images are much better suited to capture a scene's full range of absolute and relative radiance values and avoid highly lossy clipping, which can be especially problematic in very bright parts of an image.  HDR NeRF may therefore be interpreted as a volumetric HDR lighting map.

Importantly, our hybrid rendering algorithm allows us to utilize such an HDR volumetric radiance map fully.  As an HDR radiance map is particularly useful for representing the indirect bounce lighting of the scene, future work on extending such learned lighting models to direct lighting (e.g. directional or point sources that cast hard shadows) would be a promising direction. The hybrid rendering algorithm presented in this paper is a crucial ingredient to enabling such an investigation.

\mypara{Data acquisition.}
To train the HDR NeRF, we first construct a set of 32-bit HDR images of a scene, where each image is analagous to a single LDR image in the baseline NeRF formulation.  To create a single one of these HDR images, we shoot a bracketed series of LDR exposures that consists of several images (7 in our experiments) captured from a fixed camera pose.  We use a single Canon 5D MKIII with a 28mm lens, and set the camera to record images in 8-bit JPEG format.  Specifically, the camera is mounted to a tripod to minimize any minute difference in camera pose between each of the exposures in the bracket, and to minimize any optical differences between the images (e.g. depth of field, bloom, etc.) apart from raw exposure value, we only adjust the exposure duration (i.e. shutter speed) between images, while the aperture remains fixed.  The \textit{relative} difference in exposure between any consecutive images in the bracket is kept constant, though the magnitude of this difference depends on the degrees of dynamic range of the scene being captured; ideally, within the range of exposures from darkest to brightest, every pixel of the image should be ``well-exposed" in at least one of the images.  We generally captured 7 images in the bracketed exposure, with 1-2 stops difference between each image.  

\begin{wrapfigure}{r}{0.4\linewidth}
\centering
    \includegraphics[width=\linewidth]{figure/crf.png}
\caption{\textbf{Inverse Camera Response Function (CRF)} showing the recovered nonlinear function mapping from sRGB 8-bit pixel color to linear 32-bit radiance.}
\label{fig:crf_cl}
\end{wrapfigure}


\mypara{Data preprocessing.}
After capturing the scene, we preprocess the data using OpenCV.  For each bracketed exposure consisting of $n$ images taken from the same camera pose with different exposures, we align the images to ensure the best possible quality of the HDR image result, as even slight perturbations in the camera pose may cause degradation.  Then, we select a single bracketed series that is ``representative" of the lighting conditions of the full set, roughly covering the upper and lower limits of the overall dynamic range.  The representative bracketed series is used to recover the camera's nonlinear tone-mapping function, which we will refer to as the Camera Response Function (CRF) [Figure~\ref{fig:crf_cl}] using the method from \cite{debevec1997}. 

To improve computational efficiency, we recover the CRF from only one representative image, although the linear system that must be solved could theoretically incorporate pixels from \textit{all} of the bracketed series as constraints. By applying the recovered CRF uniformly to all series, we achieve consistent levels across all images.  After applying the CRF to all bracketed series, we downsample each resulting 32-bit image by a factor of $4x$.  Finally, for numerical stability during downstream training, we normalize all of the images by linearly scaling radiance values to the range of $[0, 255]$.  While this may seem similar to reducing the HDR result back to LDR, all values are scaled uniformly so the \textit{relative} differences between values are preserved, and they are \textbf{not} quantized to integer values.  The resulting HDR images are then stored as EXR files.

Note that for performing camera pose estimation using COLMAP, as is widely done in the NeRF literature, we only use a single 8-bit LDR image from each bracketed series. 
 Similarly, when training an LDR model for comparison against its HDR counterpart, we use a single image from each bracketed series, where all of the singleton images have the same exposure duration.

\mypara{HDR NeRF Implementation Details.}
Training the HDR NeRF is largely the same as training the baseline (LDR) NeRF.  In fact, the Instant-NGP implementation already supports training with 32-bit HDR images in EXR format.  We simply need to toggle flags `is\_hdr' in Instant-NGP's data loader and `linear\_colors' in the GUI.  Therefore, training is supervised purely in (scaled) linear color space, and correspondingly, the radiance component of the neural field is defined in linear color space.  Optionally, during rendering only, we may choose to apply a tonemapping function uniformly to all of the accumulated pixel radiance values to obtain the final image in sRGB color space.

\subsection{Cast Shadows on NeRF}
Reviewers said ``the more challenging and intriguing aspect is how the 3D mesh object can affect the NeRF scene(e.g., shadows, refl ections of the scene parts). The paper would look much more interesting if this part (mesh $\rightarrow$ NeRF infl uence) was studied to a deeper extent."

We query additional rays during ray-marching to cast shadows on NeRF. For each sampled point $p_t$ in NeRF, we shoot a secondary ray from $p_t$ to the light source (see the following subsection for details on estimating lighting sources). If this ray is blocked by an inserted mesh, then this $p_t$ has a shadow mask $m(p_t)=1-r_{src}$, where $r_{src}$ is the intensity of the light source. Non-blocked pixels have $m_{shadow}=1$. The contribution of this point in Eq.~\ref{eq:hdr_nerf_cl} is then 
$$T(t)\sigma(p_t) m(p_t) L_i(p_t, \omega).$$

We show in Figure~\ref{fig:shadow_ablation_cl} we can control shadow's (b) color, (c) Sharpness, and (d) direction by using different geometry and position of the light source.

\begin{figure}
\centering
\begin{tabular}{@{}c@{\hspace{1mm}}c@{\hspace{1mm}}c@{\hspace{1mm}}c@{}}
    \includegraphics[width=0.25\linewidth]{figure/family_shadow_ori.jpg} &
    \includegraphics[width=0.25\linewidth]{figure/family_shadow_light.jpg} &
    \includegraphics[width=0.25\linewidth]{figure/family_shadow_blurry.jpg} &
    \includegraphics[width=0.25\linewidth]{figure/family_shadow_direction.jpg} \\
    \small (a) Original & \small (b) Light & \small (c) Blurry & \small (d) Rotating 
\end{tabular}
\vspace{-1em}
\caption{\textbf{Shadow Casting.} }
\label{fig:shadow_ablation_cl}
\vspace{-1em}
\end{figure}


% \begin{figure}
% \centering
% \begin{tabular}{@{}c@{\hspace{1mm}}c@{\hspace{1mm}}c@{\hspace{1mm}}c@{}}
%     \includegraphics[width=0.25\linewidth]{example-image} &
%     \includegraphics[width=0.25\linewidth]{example-image} &
%     \includegraphics[width=0.25\linewidth]{example-image} &
%     \includegraphics[width=0.25\linewidth]{example-image} \\
%     % \small (c) Orignal Scene & \small (d) Inserted mesh with shadow 
% \end{tabular}
% \vspace{-1em}
% \caption{\textbf{Shadow Casting.} }
% \label{fig:shadow_ablation_cl}
% \vspace{-1em}
% \end{figure}

\subsection{Inverse Rendering for Light Source Estimation}
Sampling light sources for computing the shadow pass requires an approximate representation of the light sources (emitters) of the scene.  Note that NeRF's volume rendering formulation bakes appearance into each point in the volume rather than simulating physically based light transport.  To recover an explicit representation of light sources, we first reconstruct the geometry of the scene as a neural SDF using \emph{MonoSDF}~\cite{Yu2022MonoSDF}, from which we then extract an explicit mesh.  Then, we employ a differentiable path tracer, \emph{Mitsuba3}~\cite{Mitsuba3, Jakob2022DrJit} to estimate a UV Emission Texture for the mesh.  We follow the general approach of \cite{nimierdavid2021material}, though we customize the optimization procedure, since our goal is to estimate only the light sources, as opposed to a full BRDF estimation. Below are the details for the light source estimation.


\mypara{Geometry Reconstruction.}
Given our choice to represent light sources as area lights defined on an explicit mesh, we first need to reconstruct the geometry of the scene.  We choose to use MonoSDF \cite{Yu2022MonoSDF}, which leverages monocular geometric priors (depth and normal estimation) in the neural implicit surface reconstruction process.  Importantly, these priors especially help in reconstructing surfaces that have only a low degree of visual texture, which is very common for walls and flat tabletop surfaces.  For differentiable surface rendering, having reasonably accurate geometry is critical for achieving good convergence, as noisy geometry will tend to bias the result to bad local minima.  Empirically, MonoSDF achieves sufficiently accurate geometry for this purpose.

Once we have an optimized signed distance field, we convert it to an explicit mesh using Marching Cubes, then UV unwrap the mesh to obtain a UV texture map, using SDFStudio \cite{Yu2022SDFStudio, nerfstudio}.  This step also results in a UV texture map whose values are determined by querying the underlying MonoSDF appearance model, which we use as an albedo UV texture map.  The UV-unwrapped mesh is the input to the differentiable surface render, described below.

\mypara{Differentiable Surface Rendering.}
We implement our differentiable surface rendering optimization using Mitsuba3 \cite{Mitsuba3}, which is built on Dr. Jit \cite{Jakob2022DrJit}, a just-in-time compiler that is specialized for rendering use cases.  Our inverse rendering procedure is generally based on \cite{nimierdavid2021material}, though our specific implementation details are as follows.  The UV-unwrapped scene mesh is assigned a Principled BSDF material \cite{Burley2012PhysicallyBasedSA}, as well as an emission UV texture map, which constitute the inputs to the differentiable renderer.  The emission UV texture map, $T_{emission}$, with dimensions $(h_{tx}, w_{tx}, c_{tx})$, is the variable that we are interested in optimizing.  It is initialized uniformly with near-zero values.  The other BSDF parameters remain fixed (albedo texture map, specular transmission map with default value 1.0, and roughness map with default value 0.5).  For rendering, we use a Path-Replay Backpropagation (PRB) integrator \cite{Vicini2021PathReplay}, and limit the light transport simulation to a maximum depth of 3 (2 bounces).  This stands in contrast to differentiable rasterization approaches to inverse rendering, which are limited to a maximum depth of 2 (1 bounce), and are therefore unable to account for indirect lighting in the optimization.  We also directly render emitters (as opposed to only emitting light onto surfaces without being directly visible).


Given a set of ground-truth 32-bit HDR images $\{I_1, \cdots, I_n\}$ with dimensions $(h_{im}, w_{im}, c_{im})$ and known camera poses, our primary objective is to minimize the rendering loss (mean-squared error) between the ground truth images, and images rendered from identical camera poses.  Since the variables that we are optimizing are the emission UV texture map values, we also find that applying uniform L1 regularization to the optimization variable corresponds well to the inductive bias that the majority of the scene does not emit light, and therefore the emission UV texture map should be encouraged to be sparse.  For each optimization step $i \in [1, n]$ in a given optimization epoch, our objective is therefore to minimize the following, where $\alpha$ is a tunable hyperparameter: $$minimize\ \ \frac{1}{(h_{im} * w_{im} * c_{im})} \|I_i - \hat I_i\|^2 + \frac{\alpha}{(h_{tx} * w_{tx} * c_{tx})}|T_{emission}|$$


In addition to the rendering loss and L1 regularization in texture space, we also find that periodically clipping low values and boosting large values in the emission texture space encourages convergence toward correct results.  The motivation is that periodically during the optimization procedure (according to a tunable cadence, where we assume a default period of every 2 epochs), emission values below a given brightness threshold (also a tunable hyperparameter, with a default value of 0.2), are clipped to 0.  By assuming that very dim values are not light sources, we avoid local minima.  At the same time, values that are above this threshold are likely to be light sources, and therefore, we boost these values, in order to accelerate the optimization, since extreme emission values in the 32-bit linear color space may be arbitrarily larger than 1.  This part of the optimization should be self-correcting: values that are boosted when they shouldn't be will then be brought down in order to satisfy the rendering loss objective.  See Figure~\ref{fig:diffrender_cl} for an example of the converged result of optimizing the emission texture map.


Finally, once the optimization has converged, we post process the mesh by pruning off any triangular faces whose vertices all fall below a threshold, by looking up the brightness of each vertex in the emission UV texture map, according to that vertex's associated UV coordinates.  This results in a greatly reduced mesh that only contains faces that should emit light onto the rest of the scene, and can therefore be used as an area light for computing the shadow pass of our Hybrid Renderer.


\begin{figure}
\centering
\begin{tabular}{@{}c@{\hspace{2mm}}c@{\hspace{2mm}}c@{}}
    \includegraphics[width=0.3\linewidth]{figure/gt_images.png} &
    \includegraphics[width=0.335\linewidth]{figure/mitsuba_render.png} &
    \includegraphics[width=0.335\linewidth]{figure/emission_uv_texture.png} \\
    \small (a) Ground Truth Images & \small (b) Resulting image rendered with Mitsuba3 & \small (c) Optimized Emission UV Texture Map \\
\end{tabular}
\vspace{-2mm}
\caption{\textbf{Optimizing Emission UV Texture Map.} We optimize the (c) Emission UV Texture Map by minimizing a rendering loss objective between (a) ground truth images and (b) images rendered with Mitsuba3, a differentiable surface rendering engine.}
\label{fig:diffrender_cl}
\end{figure}

Once the light source estimation has converged, we prune faces whose emission falls below a threshold from the explicit mesh, which is necessary for efficiency, as most faces in the explicit mesh do not emit light.  The pruned mesh is then consumed by the hybrid renderer.


\subsection{Two-way coupling of the dynamics}
Reviewers also asked ``What motivated this choice given the NeRF remains static".

Although NeRF is usually used for modeling a complicated environment, in some scenarios, it can represent movable objects (e.g. a scene can be a composition of several NeRF objects~\cite{tang2022compressible}) instead of a static background. For those cases, we can get the homogenous transformation $\tt\in\mathcal{R}^{4\times 4}$ of the NeRF from simulation in each time step, which is used to inverse transform the homogenous coordinates $\tt^{-1}\cdot \pp$~\cite{pumarola2020dnerf} when querying the color/density and sampling rays in the Instant-NGP hashgrid. In Fig.~\ref{fig:game}, we control a ball to interact with a NeRF chair~\cite{mildenhall2020nerf} in real-time. Fig.~\ref{fig:ablation_dynamic_nerf_cl} and the supplementary video further shows how the collision effect changes when the ball and chair have different relative mass and velocity.


\begin{figure}
\centering
\begin{tabular}{@{}c@{\hspace{0.5mm}}c@{\hspace{0.5mm}}c@{\hspace{0.5mm}}c@{\hspace{0.5mm}}c@{\hspace{0.5mm}}c@{\hspace{0.5mm}}c@{}}
    \raisebox{3mm}{\rot{$v=5$, $m=1$}}&\includegraphics[width=0.16\linewidth]{figure/vel20/0000.jpg} &
    \includegraphics[width=0.16\linewidth]{figure/vel20/0014.jpg} &
    \includegraphics[width=0.16\linewidth]{figure/vel20/0028.jpg} &
    \includegraphics[width=0.16\linewidth]{figure/vel20/0042.jpg} &
    \includegraphics[width=0.16\linewidth]{figure/vel20/0056.jpg} &
    \includegraphics[width=0.16\linewidth]{figure/vel20/0070.jpg} \\
    \raisebox{3mm}{\rot{$v=5$, $m=25$}}&\includegraphics[width=0.16\linewidth]{figure/mass125/0000.jpg} &
    \includegraphics[width=0.16\linewidth]{figure/mass125/0014.jpg} &
    \includegraphics[width=0.16\linewidth]{figure/mass125/0028.jpg} &
    \includegraphics[width=0.16\linewidth]{figure/mass125/0042.jpg} &
    \includegraphics[width=0.16\linewidth]{figure/mass125/0056.jpg} &
    \includegraphics[width=0.16\linewidth]{figure/mass125/0070.jpg} \\
    \raisebox{3mm}{\rot{$v=1$, $m=1$}}&\includegraphics[width=0.16\linewidth]{figure/vel05/0000.jpg} &
    \includegraphics[width=0.16\linewidth]{figure/vel05/0014.jpg} &
    \includegraphics[width=0.16\linewidth]{figure/vel05/0028.jpg} &
    \includegraphics[width=0.16\linewidth]{figure/vel05/0042.jpg} &
    \includegraphics[width=0.16\linewidth]{figure/vel05/0056.jpg} &
    \includegraphics[width=0.16\linewidth]{figure/vel05/0070.jpg} \\
    % \small (c) Orignal Scene & \small (d) Inserted mesh with shadow 
\end{tabular}
\vspace{-1em}
\caption{\textbf{Ablation static for different initial velocities and relative masses.} Changing the velocities $v$ and the masses $m$ of the ball, the NeRF chair will have different motion after being hit by the ball.}
\label{fig:ablation_dynamic_nerf_cl}
\vspace{-1em}
\end{figure}
